A Quantum Algorithm for Computing All Diagnoses of a Switching Circuit

Faults are stochastic by nature while most man-made systems, and especially computers, work deterministically. This necessitates the linking of probability theory with mathematical logics, automata, and switching circuit theory. This paper provides such a connecting via quantum information theory which is an intuitive approach as quantum physics obeys probability laws. In this paper we provide a novel approach for computing diagnosis of switching circuits with gate-based quantum computers. The approach is based on the idea of putting the qubits representing faults in superposition and compute all, often exponentially many, diagnoses simultaneously. We empirically compare the quantum algorithm for diagnostics to an approach based on SAT and model-counting. For a benchmark of combinational circuits we establish an error of less than one percent in estimating the true probability of faults.

==> figures/pgflibraryref.code.tex <==
\makeatletter

\ctikzset{thickness/.initial=2}
\ctikzset{color/.initial=black}
\ctikzset{fill/.initial=white}
\pgfkeys{/tikz/color/.add code={}{\ctikzset{color={#1}}}}
\pgfkeys{/tikz/fill/.add code={}{\ctikzset{fill={#1}}}}
\pgfkeys{/tikz/refsize/.initial=1cm}

\newdimen\pgf@ref@up
\newdimen\pgf@ref@down
\newdimen\pgf@ref@left
\newdimen\pgf@ref@right

\pgf@ref@up=.15cm
\pgf@ref@down=-.15cm
\pgf@ref@left=0cm

\pgfdeclareshape{ref}{
  \nodeparts{text}

  \saveddimen{\pgf@ref@right}{\pgf@x=\pgfkeysvalueof{/tikz/refsize}}

  \anchor{center}{\pgfpointorigin}
  \anchor{west}{\pgfpoint{\pgf@ref@left}{0}}

  \anchor{in}{\pgfpoint{\pgf@ref@left}{0}}
  \anchor{out}{\pgfpoint{\pgf@ref@right}{0}}

  \anchor{text}{
    \pgf@x=1.5pt
    \pgf@y=-.5\ht\pgfnodeparttextbox
  }

  \backgroundpath{
    \pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/color}}

    \pgfscope
    \pgfsetlinewidth{2\pgflinewidth}

    \pgfpathmoveto{\pgfpoint{\pgf@ref@left}{\pgf@ref@up}}
    \pgfpathlineto{\pgfpoint{\pgf@ref@right-0.225cm}{\pgf@ref@up}}
    \pgfpathlineto{\pgfpoint{\pgf@ref@right}{0}}
    \pgfpathlineto{\pgfpoint{\pgf@ref@right-0.225cm}{\pgf@ref@down}}
    \pgfpathlineto{\pgfpoint{\pgf@ref@left}{\pgf@ref@down}}
    \pgfclosepath

    \pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/fill}}
    \pgfsetstrokecolor{black}
    \pgfusepath{draw,fill}

    \endpgfscope
  }
}

\makeatother


==> figures/pgflibrarystd_gates.code.tex <==
\makeatletter

\ctikzset{tripoles/and gate/width/.initial=1.1}
\ctikzset{tripoles/and gate/height/.initial=.8}
\ctikzset{tripoles/and gate/port width/.initial=.7}
\ctikzset{tripoles/and gate/input height/.initial=.5}
\ctikzset{tripoles/nand gate/width/.initial=1.1}
\ctikzset{tripoles/nand gate/height/.initial=.8}
\ctikzset{tripoles/nand gate/port width/.initial=.7}
\ctikzset{tripoles/nand gate/circle width/.initial=.15}
\ctikzset{tripoles/nand gate/input height/.initial=.5}
\ctikzset{tripoles/or gate/width/.initial=1.1}
\ctikzset{tripoles/or gate/height/.initial=.8}
\ctikzset{tripoles/or gate/port width/.initial=.7}
\ctikzset{tripoles/or gate/input height/.initial=.5}
\ctikzset{tripoles/or gate/input skip/.initial=.25}
\ctikzset{tripoles/or gate/aaa/.initial=.6}
\ctikzset{tripoles/or gate/bbb/.initial=.4}
\ctikzset{tripoles/or gate/ccc/.initial=.5}
\ctikzset{tripoles/or gate/ddd/.initial=.0}
\ctikzset{tripoles/nor gate/width/.initial=1.1}
\ctikzset{tripoles/nor gate/height/.initial=.8}
\ctikzset{tripoles/nor gate/port width/.initial=.7}
\ctikzset{tripoles/nor gate/input height/.initial=.5}
\ctikzset{tripoles/nor gate/input skip/.initial=.25}
\ctikzset{tripoles/nor gate/circle width/.initial=.15}
\ctikzset{tripoles/nor gate/aaa/.initial=.6}
\ctikzset{tripoles/nor gate/bbb/.initial=.4}
\ctikzset{tripoles/nor gate/ccc/.initial=.5}
\ctikzset{tripoles/nor gate/ddd/.initial=.0}
\ctikzset{tripoles/xor gate/width/.initial=1.1}
\ctikzset{tripoles/xor gate/height/.initial=.8}
\ctikzset{tripoles/xor gate/port width/.initial=.7}
\ctikzset{tripoles/xor gate/input height/.initial=.5}
\ctikzset{tripoles/xor gate/input skip/.initial=.15}
\ctikzset{tripoles/xor gate/distance/.initial=.1}
\ctikzset{tripoles/xor gate/aaa/.initial=.6}
\ctikzset{tripoles/xor gate/bbb/.initial=.4}
\ctikzset{tripoles/xor gate/ccc/.initial=.5}
\ctikzset{tripoles/xor gate/ddd/.initial=.0}
\ctikzset{tripoles/xnor gate/width/.initial=1.1}
\ctikzset{tripoles/xnor gate/height/.initial=.8}
\ctikzset{tripoles/xnor gate/port width/.initial=.7}
\ctikzset{tripoles/xnor gate/input height/.initial=.5}
\ctikzset{tripoles/xnor gate/input skip/.initial=.15}
\ctikzset{tripoles/xnor gate/distance/.initial=.1}
\ctikzset{tripoles/xnor gate/aaa/.initial=.6}
\ctikzset{tripoles/xnor gate/bbb/.initial=.4}
\ctikzset{tripoles/xnor gate/ccc/.initial=.5}
\ctikzset{tripoles/xnor gate/ddd/.initial=.0}
\ctikzset{tripoles/xnor gate/circle width/.initial=.15}
\ctikzset{bipoles/buffer/height/.initial=1}
\ctikzset{bipoles/buffer/width/.initial=1}
\ctikzset{bipoles/not gate/width/.initial=1}
\ctikzset{bipoles/not gate/height/.initial=.8}
\ctikzset{bipoles/not gate/circle width/.initial=.15}

\ctikzset{thickness/.initial=2}
\ctikzset{color/.initial=black}
\ctikzset{fill/.initial=white}
\pgfkeys{/tikz/color/.add code={}{\ctikzset{color={#1}}}}
\pgfkeys{/tikz/fill/.add code={}{\ctikzset{fill={#1}}}}

\long\def\pgfcircdeclarelogicgate#1#2{
  \pgfdeclareshape{#1 gate}{
    \savedanchor\northwest{%
      \pgf@y=\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1 gate/height}\pgf@circ@Rlen
      \pgf@y=.5\pgf@y
      \pgf@x=-\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1 gate/width}\pgf@circ@Rlen
      \pgf@x=.5\pgf@x
    }
    \anchor{in 1}{
      \pgf@y=\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1 gate/height}\pgf@circ@Rlen
      \pgf@y=.5\pgf@y
      \pgf@y=\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1 gate/input height}\pgf@y
      \pgf@x=-\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1 gate/width}\pgf@circ@Rlen
      \pgf@x=.5\pgf@x
    }
    \anchor{in 2}{
      \pgf@y=\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1 gate/height}\pgf@circ@Rlen
      \pgf@y=.5\pgf@y
      \pgf@y=\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1 gate/input height}\pgf@y
      \pgf@x=-\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1 gate/width}\pgf@circ@Rlen
      \pgf@x=.5\pgf@x
      \pgf@y=-\pgf@y
    }
    \anchor{out}{
      \northwest
      \pgf@y=0pt
      \pgf@x=-\pgf@x
    }
    \anchor{center}{
      \northwest
      \pgf@y=0pt
      \pgf@x=0pt
    }
    \backgroundpath{
      \pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/color}}

      \northwest
      \pgf@circ@res@up=\pgf@y
      \pgf@circ@res@down=-\pgf@y
      \pgf@circ@res@right=-\pgf@x
      \pgf@circ@res@left=\pgf@x

      #2

    }
  }
}

\pgfcircdeclarelogicgate{and}{
  \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}
                          {\pgfkeysvalueof{/tikz/circuitikz/tripoles/and gate/input height}\pgf@circ@res@up}}
  \pgfpathlineto{\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/and gate/port width}\pgf@circ@res@left}
                          {\pgfkeysvalueof{/tikz/circuitikz/tripoles/and gate/input height}\pgf@circ@res@up}}

  \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}
                          {\pgfkeysvalueof{/tikz/circuitikz/tripoles/and gate/input height}\pgf@circ@res@down}}
  \pgfpathlineto{\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/and gate/port width}\pgf@circ@res@left}
                          {\pgfkeysvalueof{/tikz/circuitikz/tripoles/and gate/input height}\pgf@circ@res@down}}

  \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{0pt}}
  \pgfpathlineto{\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/and gate/port width}\pgf@circ@res@right}{0pt}}

  \pgfusepath{draw}

  \pgfsetlinewidth{2\pgflinewidth}
  \pgfpathmoveto{\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/and gate/port width}\pgf@circ@res@left}{\pgf@circ@res@down}}
  \pgfpathcurveto{\pgfpoint{.0\pgf@circ@res@left}{\pgf@circ@res@down}}
                 {\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/and gate/port width}\pgf@circ@res@right}{.5\pgf@circ@res@down}}
                 {\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/and gate/port width}\pgf@circ@res@right}{0pt}}
  \pgfpathcurveto{\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/and gate/port width}\pgf@circ@res@right}{.5\pgf@circ@res@up}}
                 {\pgfpoint{.0\pgf@circ@res@left}{\pgf@circ@res@up}}
                 {\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/and gate/port width}\pgf@circ@res@left}{\pgf@circ@res@up}}
  \pgfclosepath
  \pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/fill}}
  \pgfsetstrokecolor{black}
  \pgfusepath{draw,fill}
}

\pgfcircdeclarelogicgate{nand}{
  \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/nand gate/input height}\pgf@circ@res@up}}
  \pgfpathlineto{\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/nand gate/port width}\pgf@circ@res@left}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/nand gate/input height}\pgf@circ@res@up}}

  \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/nand gate/input height}\pgf@circ@res@down}}
  \pgfpathlineto{\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/nand gate/port width}\pgf@circ@res@left}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/nand gate/input height}\pgf@circ@res@down}}

  \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{0pt}}
  \pgfpathlineto{\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/nand gate/port width}\pgf@circ@res@right}{0pt}}

  \pgfusepath{draw}

  \pgfsetlinewidth{2\pgflinewidth}

  \pgf@circ@res@step=\pgfkeysvalueof{/tikz/circuitikz/tripoles/nand gate/circle width}\pgf@circ@res@right
  \pgf@circ@res@other=\pgfkeysvalueof{/tikz/circuitikz/tripoles/nand gate/port width}\pgf@circ@res@right

  \pgfpathmoveto{\pgfpoint{-\pgf@circ@res@other}{\pgf@circ@res@down}}
  \pgfpathcurveto{\pgfpoint{.0\pgf@circ@res@left}{\pgf@circ@res@down}}
                 {\pgfpoint{\pgf@circ@res@other-\pgf@circ@res@step}{.5\pgf@circ@res@down}}
                 {\pgfpoint{\pgf@circ@res@other-\pgf@circ@res@step}{0pt}}
  \pgfpathcurveto{\pgfpoint{\pgf@circ@res@other-\pgf@circ@res@step}{.5\pgf@circ@res@up}}
                 {\pgfpoint{.0\pgf@circ@res@left}{\pgf@circ@res@up}}
                 {\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/nand gate/port width}\pgf@circ@res@left}{\pgf@circ@res@up}}
  \pgfclosepath

  \pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/fill}}
  \pgfsetstrokecolor{black}
  \pgfusepath{draw,fill}

  \pgfpathellipse{\pgfpoint{\pgf@circ@res@other-.5\pgf@circ@res@step}{0pt}}
                 {\pgfpoint{.5\pgf@circ@res@step}{0pt}}
                 {\pgfpoint{0pt}{.5\pgf@circ@res@step}}

  \pgfsetstrokecolor{black}
  \pgfusepath{draw}
}

\pgfcircdeclarelogicgate{nor}{
  \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/nor gate/input height}\pgf@circ@res@up}}
  \pgfpathlineto{\pgfpoint{(\pgfkeysvalueof{/tikz/circuitikz/tripoles/nor gate/port width}-\pgfkeysvalueof{/tikz/circuitikz/tripoles/nor gate/input skip})*\pgf@circ@res@left}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/nor gate/input height}\pgf@circ@res@up}}

  \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/nor gate/input height}\pgf@circ@res@down}}
  \pgfpathlineto{\pgfpoint{(\pgfkeysvalueof{/tikz/circuitikz/tripoles/nor gate/port width}-\pgfkeysvalueof{/tikz/circuitikz/tripoles/nor gate/input skip})*\pgf@circ@res@left}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/nor gate/input height}\pgf@circ@res@down}}

  \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{0pt}}
  \pgfpathlineto{\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/nor gate/port width}\pgf@circ@res@right}{0pt}}

  \pgfusepath{draw}

  \pgf@circ@res@other=\pgfkeysvalueof{/tikz/circuitikz/tripoles/nor gate/port width}\pgf@circ@res@right
  \pgf@circ@res@step=\pgfkeysvalueof{/tikz/circuitikz/tripoles/nand gate/circle width}\pgf@circ@res@right

  \pgfsetlinewidth{2\pgflinewidth}
  \pgfpathmoveto{\pgfpoint{-\pgf@circ@res@other}{\pgf@circ@res@up}}
  \pgfpathcurveto{\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/nor gate/aaa}\pgf@circ@res@left}{\pgf@circ@res@up}}
                 {\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/nor gate/bbb}\pgf@circ@res@left}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/nor gate/ccc}\pgf@circ@res@up}}
                 {\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/nor gate/bbb}\pgf@circ@res@left}{0pt}}
  \pgfpathcurveto{\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/nor gate/bbb}\pgf@circ@res@left}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/nor gate/ccc}\pgf@circ@res@down}}
                 {\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/nor gate/aaa}\pgf@circ@res@left}{\pgf@circ@res@down}}
                 {\pgfpoint{-\pgf@circ@res@other}{\pgf@circ@res@down}}

  \pgfpathcurveto{\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/nor gate/ddd}\pgf@circ@res@left}{\pgf@circ@res@down}}
                 {\pgfpoint{\pgf@circ@res@other-\pgf@circ@res@step}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/nor gate/ccc}\pgf@circ@res@down}}
                 {\pgfpoint{\pgf@circ@res@other-\pgf@circ@res@step}{0pt}}
  \pgfpathcurveto{\pgfpoint{\pgf@circ@res@other-\pgf@circ@res@step}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/nor gate/ccc}\pgf@circ@res@up}}
                 {\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/nor gate/ddd}\pgf@circ@res@left}{\pgf@circ@res@up}}
                 {\pgfpoint{-\pgf@circ@res@other}{\pgf@circ@res@up}}

  \pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/fill}}
  \pgfsetstrokecolor{black}
  \pgfusepath{draw,fill}

  \pgfpathellipse{\pgfpoint{\pgf@circ@res@other-.5\pgf@circ@res@step}{0pt}}
                 {\pgfpoint{.5\pgf@circ@res@step}{0pt}}
                 {\pgfpoint{0pt}{.5\pgf@circ@res@step}}

  \pgfusepath{draw}
}

\pgfcircdeclarelogicgate{or}{
  \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/or gate/input height}\pgf@circ@res@up}}
  \pgfpathlineto{\pgfpoint{(\pgfkeysvalueof{/tikz/circuitikz/tripoles/or gate/port width}-\pgfkeysvalueof{/tikz/circuitikz/tripoles/or gate/input skip})*\pgf@circ@res@left}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/or gate/input height}\pgf@circ@res@up}}

  \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/or gate/input height}\pgf@circ@res@down}}
  \pgfpathlineto{\pgfpoint{(\pgfkeysvalueof{/tikz/circuitikz/tripoles/or gate/port width}-\pgfkeysvalueof{/tikz/circuitikz/tripoles/or gate/input skip})*\pgf@circ@res@left}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/or gate/input height}\pgf@circ@res@down}}

  \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{0pt}}\pgfpathlineto{\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/or gate/port width}\pgf@circ@res@right}{0pt}}

  \pgfusepath{draw}
  \pgf@circ@res@other=\pgfkeysvalueof{/tikz/circuitikz/tripoles/or gate/port width}\pgf@circ@res@right
  \pgfsetlinewidth{2\pgflinewidth}
  \pgfpathmoveto{\pgfpoint{-\pgf@circ@res@other}{\pgf@circ@res@up}}
  \pgfpathcurveto{\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/or gate/aaa}\pgf@circ@res@left}{\pgf@circ@res@up}}
                 {\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/or gate/bbb}\pgf@circ@res@left}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/or gate/ccc}\pgf@circ@res@up}}
                 {\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/or gate/bbb}\pgf@circ@res@left}{0pt}}
  \pgfpathcurveto{\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/or gate/bbb}\pgf@circ@res@left}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/or gate/ccc}\pgf@circ@res@down}}
                 {\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/or gate/aaa}\pgf@circ@res@left}{\pgf@circ@res@down}}
                 {\pgfpoint{-\pgf@circ@res@other}{\pgf@circ@res@down}}

  \pgfpathcurveto{\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/or gate/ddd}\pgf@circ@res@left}{\pgf@circ@res@down}}
                 {\pgfpoint{\pgf@circ@res@other}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/or gate/ccc}\pgf@circ@res@down}}
                 {\pgfpoint{\pgf@circ@res@other}{0pt}}
  \pgfpathcurveto{\pgfpoint{\pgf@circ@res@other}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/or gate/ccc}\pgf@circ@res@up}}
                 {\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/or gate/ddd}\pgf@circ@res@left}{\pgf@circ@res@up}}
                 {\pgfpoint{-\pgf@circ@res@other}{\pgf@circ@res@up}}
  \pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/fill}}
  \pgfsetstrokecolor{black}
  \pgfusepath{draw,fill}
}

\pgfcircdeclarelogicgate{xor}{
  \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/xor gate/input height}\pgf@circ@res@up}}
  \pgfpathlineto{\pgfpoint{(\pgfkeysvalueof{/tikz/circuitikz/tripoles/xor gate/port width}-\pgfkeysvalueof{/tikz/circuitikz/tripoles/xor gate/input skip})*\pgf@circ@res@left}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/xor gate/input height}\pgf@circ@res@up}}

  \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/xor gate/input height}\pgf@circ@res@down}}
  \pgfpathlineto{\pgfpoint{(\pgfkeysvalueof{/tikz/circuitikz/tripoles/xor gate/port width}-\pgfkeysvalueof{/tikz/circuitikz/tripoles/xor gate/input skip})*\pgf@circ@res@left}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/xor gate/input height}\pgf@circ@res@down}}

  \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{0pt}}\pgfpathlineto{\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/xor gate/port width}\pgf@circ@res@right}{0pt}}

  \pgfusepath{draw}
  \pgf@circ@res@other=\pgfkeysvalueof{/tikz/circuitikz/tripoles/xor gate/port width}\pgf@circ@res@right
  \pgfsetlinewidth{2\pgflinewidth}
  \pgfpathmoveto{\pgfpoint{-\pgf@circ@res@other}{\pgf@circ@res@up}}
  \pgfpathcurveto{\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/xor gate/aaa}\pgf@circ@res@left}{\pgf@circ@res@up}}
                 {\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/xor gate/bbb}\pgf@circ@res@left}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/xor gate/ccc}\pgf@circ@res@up}}
                 {\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/xor gate/bbb}\pgf@circ@res@left}{0pt}}
  \pgfpathcurveto{\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/xor gate/bbb}\pgf@circ@res@left}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/xor gate/ccc}\pgf@circ@res@down}}
                 {\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/xor gate/aaa}\pgf@circ@res@left}{\pgf@circ@res@down}}
                 {\pgfpoint{-\pgf@circ@res@other}{\pgf@circ@res@down}}

  \pgfpathcurveto{\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/xor gate/ddd}\pgf@circ@res@left}{\pgf@circ@res@down}}
                 {\pgfpoint{\pgf@circ@res@other}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/xor gate/ccc}\pgf@circ@res@down}}
                 {\pgfpoint{\pgf@circ@res@other}{0pt}}
  \pgfpathcurveto{\pgfpoint{\pgf@circ@res@other}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/xor gate/ccc}\pgf@circ@res@up}}
                 {\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/xor gate/ddd}\pgf@circ@res@left}{\pgf@circ@res@up}}
                 {\pgfpoint{-\pgf@circ@res@other}{\pgf@circ@res@up}}

  \pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/fill}}
  \pgfsetstrokecolor{black}
  \pgfusepath{draw,fill}

  \def\pgf@circ@temp{-\pgfkeysvalueof{/tikz/circuitikz/tripoles/xor gate/distance}\pgf@circ@res@right+}
  \pgfpathmoveto{\pgfpoint{\pgf@circ@temp-\pgf@circ@res@other}{\pgf@circ@res@up}}

  \pgfpathcurveto{\pgfpoint{\pgf@circ@temp\pgfkeysvalueof{/tikz/circuitikz/tripoles/xor gate/aaa}\pgf@circ@res@left}{.95*\pgf@circ@res@up}}
                 {\pgfpoint{\pgf@circ@temp\pgfkeysvalueof{/tikz/circuitikz/tripoles/xor gate/bbb}\pgf@circ@res@left}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/xor gate/ccc}\pgf@circ@res@up}}
                 {\pgfpoint{\pgf@circ@temp\pgfkeysvalueof{/tikz/circuitikz/tripoles/xor gate/bbb}\pgf@circ@res@left}{0pt}}
  \pgfpathcurveto{\pgfpoint{\pgf@circ@temp\pgfkeysvalueof{/tikz/circuitikz/tripoles/xor gate/bbb}\pgf@circ@res@left}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/xor gate/ccc}\pgf@circ@res@down}}
                 {\pgfpoint{\pgf@circ@temp\pgfkeysvalueof{/tikz/circuitikz/tripoles/xor gate/aaa}\pgf@circ@res@left}{.95*\pgf@circ@res@down}}
                 {\pgfpoint{\pgf@circ@temp-\pgf@circ@res@other}{.95*\pgf@circ@res@down}}

  \pgfusepath{draw}
}

\pgfcircdeclarelogicgate{xnor}{
  \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/xnor gate/input height}\pgf@circ@res@up}}
  \pgfpathlineto{\pgfpoint{(\pgfkeysvalueof{/tikz/circuitikz/tripoles/xnor gate/port width}-\pgfkeysvalueof{/tikz/circuitikz/tripoles/xnor gate/input skip})*\pgf@circ@res@left}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/xnor gate/input height}\pgf@circ@res@up}}

  \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/xnor gate/input height}\pgf@circ@res@down}}
  \pgfpathlineto{\pgfpoint{(\pgfkeysvalueof{/tikz/circuitikz/tripoles/xnor gate/port width}-\pgfkeysvalueof{/tikz/circuitikz/tripoles/xnor gate/input skip})*\pgf@circ@res@left}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/xnor gate/input height}\pgf@circ@res@down}}

  \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{0pt}}\pgfpathlineto{\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/xnor gate/port width}\pgf@circ@res@right}{0pt}}

  \pgfusepath{draw}
  \pgf@circ@res@other=\pgfkeysvalueof{/tikz/circuitikz/tripoles/xnor gate/port width}\pgf@circ@res@right
  \pgf@circ@res@step=\pgfkeysvalueof{/tikz/circuitikz/tripoles/xnor gate/circle width}\pgf@circ@res@right

  \pgfsetlinewidth{2\pgflinewidth}
  \pgfpathmoveto{\pgfpoint{-\pgf@circ@res@other}{\pgf@circ@res@up}}
  \pgfpathcurveto{\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/xnor gate/aaa}\pgf@circ@res@left}{\pgf@circ@res@up}}
                 {\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/xnor gate/bbb}\pgf@circ@res@left}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/xnor gate/ccc}\pgf@circ@res@up}}
                 {\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/xnor gate/bbb}\pgf@circ@res@left}{0pt}}
  \pgfpathcurveto{\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/xnor gate/bbb}\pgf@circ@res@left}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/xnor gate/ccc}\pgf@circ@res@down}}
                 {\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/xnor gate/aaa}\pgf@circ@res@left}{\pgf@circ@res@down}}
                 {\pgfpoint{-\pgf@circ@res@other}{\pgf@circ@res@down}}

  \pgfpathcurveto{\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/xnor gate/ddd}\pgf@circ@res@left}{\pgf@circ@res@down}}
                 {\pgfpoint{\pgf@circ@res@other-\pgf@circ@res@step}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/xnor gate/ccc}\pgf@circ@res@down}}
                 {\pgfpoint{\pgf@circ@res@other-\pgf@circ@res@step}{0pt}}
  \pgfpathcurveto{\pgfpoint{\pgf@circ@res@other-\pgf@circ@res@step}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/xnor gate/ccc}\pgf@circ@res@up}}
                 {\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/xnor gate/ddd}\pgf@circ@res@left}{\pgf@circ@res@up}}
                 {\pgfpoint{-\pgf@circ@res@other}{\pgf@circ@res@up}}

  \pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/fill}}
  \pgfsetstrokecolor{black}
  \pgfusepath{draw,fill}

  \def\pgf@circ@temp{-\pgfkeysvalueof{/tikz/circuitikz/tripoles/xnor gate/distance}\pgf@circ@res@right+}
  \pgfpathmoveto{\pgfpoint{\pgf@circ@temp-\pgf@circ@res@other}{\pgf@circ@res@up}}

  \pgfpathcurveto{\pgfpoint{\pgf@circ@temp\pgfkeysvalueof{/tikz/circuitikz/tripoles/xnor gate/aaa}\pgf@circ@res@left}{.95*\pgf@circ@res@up}}
                 {\pgfpoint{\pgf@circ@temp\pgfkeysvalueof{/tikz/circuitikz/tripoles/xnor gate/bbb}\pgf@circ@res@left}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/xnor gate/ccc}\pgf@circ@res@up}}
                 {\pgfpoint{\pgf@circ@temp\pgfkeysvalueof{/tikz/circuitikz/tripoles/xnor gate/bbb}\pgf@circ@res@left}{0pt}}
  \pgfpathcurveto{\pgfpoint{\pgf@circ@temp\pgfkeysvalueof{/tikz/circuitikz/tripoles/xnor gate/bbb}\pgf@circ@res@left}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/xnor gate/ccc}\pgf@circ@res@down}}
                 {\pgfpoint{\pgf@circ@temp\pgfkeysvalueof{/tikz/circuitikz/tripoles/xnor gate/aaa}\pgf@circ@res@left}{.95*\pgf@circ@res@down}}
                 {\pgfpoint{\pgf@circ@temp-\pgf@circ@res@other}{.95*\pgf@circ@res@down}}

  \pgfusepath{draw}

  \pgfpathellipse{\pgfpoint{\pgf@circ@res@other-.5\pgf@circ@res@step}{0pt}}
                 {\pgfpoint{.5\pgf@circ@res@step}{0pt}}
                 {\pgfpoint{0pt}{.5\pgf@circ@res@step}}

  \pgfusepath{draw}
}

\pgfdeclareshape{not gate}{
  \anchor{center}{\pgfpointorigin}
  \savedanchor\northwest{
    \pgf@y=\pgfkeysvalueof{/tikz/circuitikz/bipoles/not gate/height}\pgf@circ@Rlen
    \pgf@y=.5\pgf@y
    \pgf@x=-\pgfkeysvalueof{/tikz/circuitikz/bipoles/not gate/width}\pgf@circ@Rlen
    \pgf@x=.5\pgf@x
  }
  \anchor{in}{
    \northwest
    \pgf@y=0pt
  }
  \anchor{out}{
    \northwest
    \pgf@y=0pt
    \pgf@x=-\pgf@x
  }
  \backgroundpath{
    \pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/color}}

    \northwest
    \pgf@circ@res@up=\pgf@y
    \pgf@circ@res@down=-\pgf@y
    \pgf@circ@res@right=-\pgf@x
    \pgf@circ@res@left=\pgf@x

    \pgf@circ@res@other=\pgfkeysvalueof{/tikz/circuitikz/bipoles/not gate/circle width}\pgf@circ@res@right

    \pgfscope
    \pgfsetlinewidth{2\pgflinewidth}
    \pgftransformxshift{.7\pgf@circ@res@left}
    \pgf@circ@res@step=\pgf@circ@res@right
    \advance\pgf@circ@res@step by -\pgf@circ@res@left
    \pgf@circ@res@step=.7\pgf@circ@res@step

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@step-\pgf@circ@res@other}{0pt}}
    \pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@down}}
    \pgfclosepath
    \pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/fill}}
    \pgfsetstrokecolor{black}
    \pgfusepath{draw,fill}

    \pgfpathellipse{\pgfpoint{\pgf@circ@res@step-.5\pgf@circ@res@other}{0pt}}
                   {\pgfpoint{.5\pgf@circ@res@other}{0pt}}
                   {\pgfpoint{0pt}{.5\pgf@circ@res@other}}
    \pgfsetcolor{white}
    \pgfsetstrokecolor{black}
    \pgfusepath{draw,fill}
    \endpgfscope

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{0pt}}
    \pgfpathlineto{\pgfpoint{.7\pgf@circ@res@left}{0pt}}

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{0pt}}
    \pgfpathlineto{\pgfpoint{.7\pgf@circ@res@right}{0pt}}

    \pgfusepath{draw}
  }
}

\pgfdeclareshape{buffer gate}{
  \anchor{center}{\pgfpointorigin}
  \savedanchor\northwest{%
    \pgf@y=\pgfkeysvalueof{/tikz/circuitikz/bipoles/not gate/height}\pgf@circ@Rlen
    \pgf@y=.5\pgf@y
    \pgf@x=-\pgfkeysvalueof{/tikz/circuitikz/bipoles/not gate/width}\pgf@circ@Rlen
    \pgf@x=.5\pgf@x
  }
  \savedanchor\left{%
    \pgf@y=0pt
  }
  \anchor{in}{
    \northwest
    \pgf@y=0pt
  }
  \anchor{out}{
    \northwest
    \pgf@y=0pt
    \pgf@x=-\pgf@x
  }
  \backgroundpath{
    \pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/color}}

    \northwest
    \pgf@circ@res@up=\pgf@y
    \pgf@circ@res@down=-\pgf@y
    \pgf@circ@res@right=-\pgf@x
    \pgf@circ@res@left=\pgf@x

    \pgf@circ@res@other=\pgfkeysvalueof{/tikz/circuitikz/bipoles/not gate/circle width}\pgf@circ@res@right

    \pgfscope
    \pgfsetlinewidth{2\pgflinewidth}
    \pgftransformxshift{.7\pgf@circ@res@left}
    \pgf@circ@res@step=\pgf@circ@res@right
    \advance\pgf@circ@res@step by -\pgf@circ@res@left
    \pgf@circ@res@step=.7\pgf@circ@res@step

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@step-\pgf@circ@res@other}{0pt}}
    \pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@step-\pgf@circ@res@other}{0pt}}
    \pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/fill}}
    \pgfsetstrokecolor{black}
    \pgfusepath{draw,fill}
    \endpgfscope

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{0pt}}
    \pgfpathlineto{\pgfpoint{.7\pgf@circ@res@left}{0pt}}

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{0pt}}
    \pgfpathlineto{\pgfpoint{.5\pgf@circ@res@right}{0pt}}

    \pgfusepath{draw}

  }
}

\pgfdeclareshape{tristate buffer gate}{
  \anchor{center}{\pgfpointorigin}
  \savedanchor\northwest{
    \pgf@y=\pgfkeysvalueof{/tikz/circuitikz/bipoles/not gate/height}\pgf@circ@Rlen
    \pgf@y=.5\pgf@y
    \pgf@x=-\pgfkeysvalueof{/tikz/circuitikz/bipoles/not gate/width}\pgf@circ@Rlen
    \pgf@x=.5\pgf@x
  }
  \savedanchor\left{
    \pgf@y=0pt
  }
  \anchor{in}{
    \northwest
    \pgf@y=0pt
  }
  \anchor{en}{
    \northwest
    \pgf@x=0pt
  }
  \anchor{out}{
    \northwest
    \pgf@y=0pt
    \pgf@x=-\pgf@x
  }
  \anchor{center}{
    \pgfpointorigin
  }
  \backgroundpath{
    \pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/color}}

    \northwest
    \pgf@circ@res@up=\pgf@y
    \pgf@circ@res@down=-\pgf@y
    \pgf@circ@res@right=-\pgf@x
    \pgf@circ@res@left=\pgf@x

    \pgf@circ@res@other=\pgfkeysvalueof{/tikz/circuitikz/bipoles/not gate/circle width}\pgf@circ@res@right

    \pgfscope
    \pgfsetlinewidth{2\pgflinewidth}
    \pgftransformxshift{.7\pgf@circ@res@left}
    \pgf@circ@res@step=\pgf@circ@res@right
    \advance\pgf@circ@res@step by -\pgf@circ@res@left
    \pgf@circ@res@step=.7\pgf@circ@res@step

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@step-\pgf@circ@res@other}{0pt}}
    \pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@step-\pgf@circ@res@other}{0pt}}
    \pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/fill}}
    \pgfsetstrokecolor{black}
    \pgfusepath{draw,fill}
    \endpgfscope

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{0pt}}
    \pgfpathlineto{\pgfpoint{.7\pgf@circ@res@left}{0pt}}

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{0pt}}
    \pgfpathlineto{\pgfpoint{.5\pgf@circ@res@right}{0pt}}

    \pgfpathmoveto{\pgfpoint{0pt}{.45\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@up}}

    \pgfusepath{draw}
  }
}

\makeatother

